SAFER: Safe Collision Avoidance using Focused and Efficient Trajectory Search with Reinforcement Learning

Collision avoidance is key for mobile robots and agents to operate safely in the real world. In this work we present SAFER, an efficient and effective collision avoidance system that is able to improve safety by correcting the control commands sent by an operator. It combines real-world reinforcement learning (RL), search-based online trajectory planning, and automatic emergency intervention, e.g. automatic emergency braking (AEB). The goal of the RL is to learn an effective corrective control action that is used in a focused search for collision-free trajectories, and to reduce the frequency of triggering automatic emergency braking. This novel setup enables the RL policy to learn safely and directly on mobile robots in a real-world indoor environment, minimizing actual crashes even during training. Our real-world experiments show that, when compared with several baselines, our approach enjoys a higher average speed, lower crash rate, less emergency intervention, smaller computation overhead, and smoother overall control.

==> algorithms/algo.tex <==
\begin{algorithm}[t!]
\caption{Training Algorithm}
\begin{algorithmic}[1]
\State Initialize experience buffer $\mathcal{D} \leftarrow \emptyset$
\State Randomly initialize RL network parameters $\theta$
\For{learning epochs}
    \State $(v_{\rm ref}, \omega_{\rm ref}) \leftarrow$ control command
    \State $s_t \leftarrow$ \{sensor scans, $v, w, v_{\rm ref}, \omega_{\rm ref}$\}
    \If{maximum braking required}
        \State $\sigma_t \leftarrow 1$, perform maximum braking 
        \State $a_t, (v_c, \omega_c) \leftarrow {\rm Null}, (-v_{\rm max}, 0)$
    \Else
        \State $\sigma_t \leftarrow 0$, do not perform maximum braking 
        \If{collision avoidance required}
            \State $a_t \leftarrow [throttle, turn] \leftarrow$ RL policy network
            \State $(v_c, \omega_c) \leftarrow$ targeted search with $\{s_{t}, a_{t}\}$
        \Else
            \State $a_t, (v_c, \omega_c) \leftarrow {\rm Null}, (v_{\rm ref}, \omega_{\rm ref})$
        \EndIf
    \EndIf
    \If{$a_{t-1}$ not ${\rm Null}$}
        \State $r_{t-1}\leftarrow$ eq.~\eqref{eq:reward} with $\{s_{t-1}, a_{t-1}, \sigma_t\}$
        \State $\mathcal{D} \leftarrow \{s_{t-1}, a_{t-1}, r_{t-1}, \sigma_t\}$
    \EndIf
    \State command robot with $(v_c, \omega_c)$
\State use $\mathcal{D}$ to update $\theta$ using RL
\EndFor
\end{algorithmic}
\label{procedure:LAMB}
\end{algorithm}


==> fig_tex/glass.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/glass.png}
    \caption{Qualitative results for difficult scenarios of glass obstacles. Upstream control has goal intention (green star) of navigating robot through glass due to lack of Lidar returns for the see-through surface (circled in green). We show the trajectory search space for both the traditional search method and our RL-guided search. Our method produces a more effective search space excluding trajectories that collide with glass, learning to leverage sparse Ultrasonic sensory input.}
    \label{fig:glass}
\end{figure}

==> fig_tex/highlevel.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/highlevel.png}
    \caption{Diagram shows the safety system performing a path search to control robot out of a potential collision, while also heading towards the goal. The RL Guided Search is able to find the optimal path with a much smaller search space.}
    \label{fig:highlevel}
\end{figure}

==> fig_tex/human.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/human.png}
    \caption{Qualitative results for obstacle avoidance in the presence of a human. The human is circled in green and is shown walking into the path of the robot, as time elapses going down the column of plots. We show the trajectory search space for both the traditional search method and our RL-guided search. Our RL-guided search method is able to adapt the search space bounds to effectively include trajectories that plan a path away from the human, while still attempting to make progress toward the goal (green star). The traditional search is unable to adapt and showing same larger search spaces.}
    \label{fig:human}
\end{figure}

==> fig_tex/mainfigure.tex <==
\begin{figure*}[t!]
    \vspace{0mm}
    \centering
    %\includegraphics[width=1.0\textwidth]{figures/mainfigure.png}
    \includegraphics[width=0.9\textwidth]{figures/illustration.jpg}
    \vspace{-4mm}
    \caption{a) Diagram of our collision avoidance system, and our robotic platform with a self-balancing base with differential drive, an onboard Linux computer (Nvidia Jetson NX), a 2D $360^\circ$ lidar scanner (RPLidar A3), and an ultrasonic sensor array. b) Our training and testing environments. c)  Illustration of the RL-guided search with learned search heuristics.}
    %\caption{\color{red} Figure in (A) depicts the logical flow of our bypass safety system. Images in (B) show our robotic platform with a self-balancing base with differential drive, an onboard linux computer, a 360-degree lidar scanner, and an ultrasonic sensor array. We also show parts of our office training environment, and testing environment which contains different structures and layout. Figure (C) shows our reinforcement learning setup, with a centralized training server that receives collected experiences from robots, and distributed robots receiving updated policy network weights for running inference and collecting experience. The received experiences by the server are stored into a shared replay buffer as samples to train and improve the policy network under Soft Actor Critic (SAC)~\cite{haarnoja2018soft}. The server sends updated networks to the robotic agents at fixed intervals. Network diagram (D) displays the policy and the critic network with 1D convolution layers denoted with (num\_kernels, kernel\_size, stride, padding), and fully connected layers denoted with the layer size. The state $s_t$ consists of 360 point lidar scan ($l$), 3 way ultrasonic sensor scan ($u$), robot linear velocity ($v$), robot angular velocity ($w$), robot upstream throttle command ($throttle$), and robot upstream turn command ($turn$). The policy network takes in the state $s_t$ and outputs actions $a_t$ as four window bounds for the search window: $a_t := \pi_{out} := [b_0, b_1, b_2, b_3]$. The critic network (Q-network) takes in the state $s_t$ and action $a_t$ and outputs a single Q value. Diagram (E) shows how the RL Guided Search is able to find the optimal path with a much smaller, and more favorable search space in comparison to the standard search.}
    \label{fig:mainfigure}
    \vspace{-5mm}
\end{figure*}

==> fig_tex/network.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/network.png}
    \vspace{-3mm}
    \caption{The policy and the critic network. The state $s_t$ consists of 360 point Lidar scan ($l$), 3 way Ultrasonic sensor scan ($u$), robot linear velocity ($v$), robot angular velocity ($w$), robot upstream throttle command ($throttle$), and robot upstream turn command ($turn$). The policy network takes in the state $s_t$ and outputs actions $a_t$ as four window bounds for the search window: $a_t := \pi_{out} := [b_0, b_1, b_2, b_3]$. The critic network (Q-network) takes in the state $s_t$ and action $a_t$ and outputs a single Q value.}
    \label{fig:network}
\end{figure}

==> fig_tex/offices.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/offices.png}
    \caption{Image demonstrating part of our office training environment (left), and office test environment for generalization (right). We picked parts of the office that are vastly different in order to demonstrate the robustness of our method. The test environment contains many cubicles, and structures not seen in our training environment.}
    \label{fig:offices}
\end{figure}

==> fig_tex/reward_train.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/reward_train.png}
    \caption{Training plot comparing the reward achieved per training step in our experimental setup, for both the Pure RL and RL-Guided Search methods. Our learned search outperforms the pure RL policy by a large margin during training, and is able to effectively learn an optimal policy in just over 5000 training steps, or around 2.5 hours of training data on our robotic platform.}
    \label{fig:reward_train}
\end{figure}

==> fig_tex/robot.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/robot_office.png}
    \caption{Our robotic platform (left image), with a self-balancing robotic base with differential drive, an onboard linux compute (serial communication to control the robot base by body velocities), a 360-degree Lidar scanner, and a Ultrasonic sensor array. Images showing parts of our office training environment (upper right) and testing environment for generalization (lower right); the test environment contains cubicles and structures not seen in our training environment.}
    \label{fig:robot}
\end{figure}

==> fig_tex/static.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/static.png}
    \caption{Qualitative results for obstacle avoidance against static obstacles like walls and furniture. We show the trajectory search space for both the traditional DWA search method and our RL-Guided (bounded) search. Our RL-Guided search method outputs far fewer trajectories for the search, proving to be more efficient. It also outputs trajectories that are more likely to be optimal, considering progress made toward the goal (green star), and collisions with nearby obstacles. The traditional search is unable to adapt and always has the same large search space.}
    \label{fig:static}
\end{figure}

==> fig_tex/train_setup.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/distributed_training.png}
    \vspace{-3mm}
    \caption{Our reinforcement learning setup. A centralized training server that receives collected experiences from robots, and distributed robots receiving updated policy network weights for running inference and collecting experience. The received experiences by the server are stored into a shared replay buffer as samples to train and improve the policy network under Soft Actor Critic (SAC)~\cite{haarnoja2018soft}. The server sends updated networks to the robotic agents at fixed intervals. This setup operates over a WiFi-network connection, allowing multiple robots to be part of the training cycle to increase the amount of experience collection, and accelerate training.}
    \label{fig:train_setup}
\end{figure}

==> sections/method_old.tex <==
\vspace{-1mm}
\section{Method}
\vspace{-1mm}

We present our collision avoidance system in Fig.~\ref{fig:mainfigure} (a), noting that our method runs in parallel with upstream tasks, such as navigation planning and human control. Our approach takes as input the robot state from odometry, the lidar and ultrasonic scans, and the control command from the upstream tasks. The output is a corrective control command to the upstream reference tasks, which avoids collision and provides favorable behavior (fast speed, smooth control, etc.). There are two stages within our collision avoidance: {\em maximum braking and collision avoidance checks} (details in Sec.~\ref{subsec:safety_check}) and {\em RL collision avoidance policy} (details in Sec.~\ref{subsec:RL_policy_search}). In the first stage, we determine whether the robot requires maximum braking, or a corrective control command through our RL policy. In the second stage, we apply our
RL policy to output corrective control commands with the goal of 1) reducing the frequency of emergency braking interventions and 2) avoiding collision effectively. 

\subsection{Maximum Braking and Collision Avoidance}
\label{subsec:safety_check}
  According to the robot's current state and the surrounding obstacles, we first check whether emergency intervention or collision avoidance is necessary, and apply corrective action to the upstream control commands. If emergency intervention is required, we apply maximum braking to bring the robot to a complete stop. If emergency braking is not required, but collision avoidance is, we apply a corrective control command using our RL policy. If neither emergency braking nor collision avoidance is required, our system maintains the upstream control. In the following, we first define collision, then discuss how we determine whether to apply emergency braking or collision avoidance through RL.
 
 \underline{Collision.} We define $\mathbb{E}(\mathbf{x})\in\mathbb{R}^2$ as the set of points in 2D space by the robot's shape at state $\mathbf{x}$. A collision occurs between the robot's trajectory $\mathbf{traj}(v, \omega, \Delta t)$ and the set of obstacles $\mathbb{O}_s\subset\mathbb{R}^2$ if:
\begin{equation}
    \bigcup_{\mathbf{x}\in \mathbf{traj}(v, \omega, \Delta t)}(\mathbb{E}(\mathbf{x}) \cap \mathbb{O}_s) \neq \emptyset.
\label{eq:collision}
\end{equation}
 
 \underline{Emergency Braking} We adopt maximum braking control when the robot's trajectory along the plan-ahead time $t_p$, denoted as $\mathbf{traj}(v, \omega, t_p)$, collides with obstacles, formulated as {\small $\bigcup_{\mathbf{x}\in \mathbf{traj}(v, \omega, t_p)}\mathbb{E}(\mathbf{x}) \cap \mathbb{O}_s \neq \emptyset$}.
 
 \underline{Collision Avoidance} If maximum braking is not required, then we expand the plan-ahead time to $\beta t_p$, where $\beta > 1$, to see if the robot collides with obstacles that are further away. Larger values of $\beta$ result in earlier (and more) collision avoidance intervention, and is a hyper-parameter that we set to $\beta = 2$\footnote{We found $\beta = 2$ to be a good balance to avoid emergency braking, and minimize collision avoidance intervention to upstream control.}. It can be formulated as {\small $\bigcup_{\mathbf{x}\in \mathbf{traj}(v, \omega, \beta t_p)}\mathbb{E}(\mathbf{x}) \cap \mathbb{O}_s \neq \emptyset$}. If there is a collision, then we use our RL policy to output a corrective control command. 
 
\subsection{RL Collision Avoidance Policy}
\label{subsec:RL_policy_search}
Our RL policy is inspired by the Dynamic Window Approach (DWA)~\cite{fox1997dynamic}. The DWA approach defines a dynamic window $W=[v_{\rm lower}, v_{\rm upper}] \times [\omega_{\rm lower}, \omega_{\rm upper}]$ identifying the set formed by the Cartesian product of values in the range between lower and upper linear velocity, and angular velocity values. DWA then performs an exhaustive search for a control command $(v_c, \omega_c)$ $\in$ $W$ that minimizes a defined cost. Alternatively, our approach improves upon this by using the output of an RL policy to guide DWA, allowing us to perform a smaller targeted search to find the optimal control. In the following, we show the traditional search space (dynamic window) in DWA, discuss the RL policy and reward, and finally discuss our RL-guided search.

\underline{Standard Dynamic Window.} In the DWA approach~\cite{fox1997dynamic}, the standard dynamic window $W$ is defined using the current robot velocity $(v,\omega)$, the maximum linear and angular acceleration $(a_{\rm max}^v, a_{\rm max}^\omega)$, and the robot reaction-time $t_r$:
\begin{equation}
\begin{aligned}
W = [max(v-a_{\rm max}^vt_r, -v_{\rm max}), min(v+a_{\rm max}^vt_r, v_{\rm max})] \times 
\\
[max(\omega-a_{\rm max}^\omega t_r, -\omega_{\rm max}), min(\omega+a_{\rm max}^\omega t_r, \omega_{\rm max})]. 
\label{eq:window}
\end{aligned}
\end{equation}
Searching in $W$ can be inefficient since the ranges between the lower and upper velocities can be large, and small search granularity is needed to find good solutions. To be specific, in DWA we typically consider a search consisting of $n_v$ linear and $n_\omega$ angular velocity control commands inside of the window $W$, which yields a search space of $n_v*n_\omega$ trajectories. The granularity of such a search (at maximum) is $2a_{\rm max}^vt_r / n_v$ for linear velocity, and $2a_{\rm max}^\omega t_r / n_\omega$ for angular velocity.

\underline{RL Policy and Reward.} We consider a distributed RL training setup with the soft actor critic (SAC)~\cite{haarnoja2018soft} approach. Our robots collect experiences and send them to a central training server, and the training server uses these experiences to train and update the actor's policy network, as well as the critic and critic target networks. The training server sends all robots the updated actor network after a fixed number of training steps. The following figures present the overall setup and network specifications:
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/distributed_rl.jpg}
\end{center}
\vspace{-5mm}
\begin{center}
\includegraphics[width=0.75\linewidth]{figures/network_spec.pdf}
\vspace{-3mm}
\end{center}

For each time step, $s_t$ represents the input to the policy and the critic network, consisting of lidar and ultrasonic scans, robot's linear and angular velocity, and the control commands from the upstream task: $s_t = [l_0, l_1, \cdots, l_{359}, u_{-45}, u_0, u_{45}, v, \omega, v_{\rm ref}, \omega_{\rm ref}]$. 

$a_t$ is the output of the policy network and also part of the input to the critic network: $a_t = [throttle, turn] \in [-1, 1]$

$r_t$ is our reward function. Since we aim to learn corrective control commands that can 1) reduce the number of maximum braking interventions and 2) avoid collision effectively, we compose $r_t$ to be
\begin{equation}
\small
r_t = -\lambda_1 \sigma_{t+1} - \lambda_2 J(v_c, \omega_c),  
\label{eq:reward}
\end{equation}
where $\lambda_1, \lambda_2$ are hyper-parameters\footnote{In our design, $\lambda_1=35, \lambda_2=10$.}, $\sigma_{t+1}$ indicates whether maximum braking was performed in the next time step, and $J(v_c, \omega_c)$ is the cost of the control command $(v_c, \omega_c)$. Precisely, we define $J(v_c, \omega_c)$ as
\begin{equation}
\small
\begin{aligned}
   J(v_c, \omega_c) &= \mathrm{c}_1(v_{\rm max} - v_c) + \mathrm{c}_2 (|v_c-v_{\rm ref}| + |\omega_c-\omega_{\rm ref}|)\\
   & \quad+ \mathrm{c}_3\frac{1}{\operatorname{dist}\big(\mathbb{O}_s, \mathbf{traj}(v_c, \omega_c, \beta t_p)\big)},
\label{eq:cost}
\end{aligned}
\end{equation}
where $c_1, c_2, c_3$ are hyper-parameters\footnote{In our settings, $c_1=0.4, c_2=0.2, c_3=0.4$},  $(v_{\rm max} - v_c)$ encourages the corrective linear velocity to be fast, $(|v_c-v_{\rm ref}| + |\omega_c-\omega_{\rm ref}|)$ minimizes the deviation of corrective control commands from upstream control commands, and $\frac{1}{\rm dist(\cdot)}$ encourages the robot to stay away from obstacles with $\operatorname{dist}(\mathbb{O}_s, \mathbf{traj})$ distance between the robot's trajectory and the obstacles:
{\small $$
 \operatorname{dist}(\mathbb{O}_s, \mathbf{traj}) = \min_{\forall (x_s, y_s) \in \mathbb{O}_s, (\hat{x}, \hat{y})\in\mathbf{x}\in\mathbf{traj}} \lVert (\hat{x}, \hat{y}) - (x_s, y_s) \rVert .
$$}

\input{algorithms/algo}

\underline{RL-guided Search.} After we obtain $throttle, turn$ from the RL policy network, we scale the output as $[v_s, \omega_s]=[throttle*v_{\rm max}, turn*\omega_{\rm max}]$. We then check to make sure that the scaled output $[v_s, \omega_s]$ is feasible and lies within the dynamic window $W=[v_{\rm lower}, v_{\rm upper}] \times [\omega_{\rm lower}, \omega_{\rm upper}]$ as defined in equation~\ref{eq:window}. If $[v_s, \omega_s] \notin W$, then we threshold the scaled output to fit into $W$:
\begin{equation}
\small
[max(min(v_s, v_{\rm upper}), v_{\rm lower}), max(min(\omega_s, \omega_{\rm upper}), \omega_{\rm lower})]
\label{eq:rlcommand}
\end{equation}
Next we perform a targeted search around the scaled RL action using parameters $\gamma \in (0, 1)$ and $\delta \in (0, 1)$, inspired by the traditional DWA window discussed in equation~\ref{eq:window}. Our search picks the corrective control $v_c, \omega_c$ that minimizes $J(v_c, \omega_c)$ in equation~\ref{eq:cost}. We create a search window around $[v_s, \omega_s]$ that is $\gamma$ times the size of the standard window in~\ref{eq:window}. Our $[v_{\rm lower}, v_{\rm upper}] \times [\omega_{\rm lower}, \omega_{\rm upper}]$ becomes:
\begin{equation}
\begin{aligned}
[max(v_s-\gamma a_{\rm max}^vt_r, -v_{\rm max}), min(v_s+\gamma a_{\rm max}^vt_r, v_{\rm max})] \times 
\\
[max(\omega_s-\gamma a_{\rm max}^\omega t_r, -\omega_{\rm max}), min(\omega_s+ \gamma a_{\rm max}^\omega t_r, \omega_{\rm max})]. 
\label{eq:reduced_window}
\end{aligned}
\end{equation}
We then sample $\delta n_v$ linear velocities and $\delta n_\omega$ angular velocities from the smaller window, resulting in a total of $\delta^2 n_v n_\omega$ trajectories being searched. This also yields a search granularity (at maximum) of $2\gamma a_{\rm max}^vt_r / \delta n_v$ for linear velocity, and $2\gamma a_{\rm max}^\omega t_r / \delta n_\omega$ for angular velocity, meaning the granularity is $\gamma / \delta$ compared to standard. To summarize, our targeted search window is $1 / \gamma$ times smaller, and we sample $1 / \delta^2$ less trajectories. In the experiments section we show that this targeted search outperforms standard DWA search in finding an optimal control for collision avoidance, in a small fraction of the time.

\subsection{Tuning Collision Avoidance Hyperparameters}
In order to aid the reader in understanding how to tune the more important collision avoidance parameters in our work, $[\beta, n_v, n_\omega, \gamma, \delta]$, we provide a brief discussion. 
\begin{itemize}
    \item $\beta>1$ controls the planning look-ahead multiplier. Larger settings causes the RL-guided search to be triggered more often for collision avoidance, which can be desirable to a certain extent; too large of a setting can negatively affect the human control experience due to being overly conservative. We recommend tuning this parameter based on the desired level of collision avoidance interruption to user control. We set $\beta=2$.
    \item $n_v, n_\omega$ determine how many linear and angular velocities are sampled from the dynamic window, resulting in $n_v n_\omega$ samples. We maximize the values of $n_v, n_\omega$ up to the point where the standard DWA search achieves a planning cycle latency of the desired $t_r$ (100ms in our setting). Depending on the robotic platform, one can increase the value of $n_v$ compared to $n_\omega$ or vice-versa if the window size is larger in either direction. 
    \item $\gamma, \delta \in (0, 1)$ control the size of the targeted RL search. $\delta$ should be set such that the search time $t_{search}$ resulting from the number of samples $\delta^2 n_v n_\omega$ offsets the inference time of the RL policy $t_{\pi}$; $t_{search} \leq t_r - t_{\pi}$. $\gamma$ is then set to achieve the desired search granularity compared to the standard DWA search $\gamma / \delta$, ideally $\gamma / \delta \leq 1$ (more granular). 
\end{itemize}

\input{tbl_tex/old_table}
\input{tbl_tex/generalization}


==> sections/old_abstract.tex <==
Obstacle avoidance is a challenging and critical task in indoor mobile robotics. A common method for ensuring safety against obstacle collision in real world environments is the Automated Emergency Braking (AEB) systems, typically seen in driving vehicles. These approaches often fall short in achieving optimal behavior in an environment, and can cause the user experience to suffer. Other popular methods that leverage heuristic search often frame obstacle avoidance as one of the optimization terms in a larger trajectory optimization problem. However this does not consider safety as the primary goal due to the trade-off between the optimization terms. Using learning-based techniques, such as Reinforcement Learning, has become appealing because it can enable robots to learn a representation that allows for generalize-able and adaptable behavior. However there is a significant barrier in using Reinforcement Learning based approaches in robotic obstacle avoidance due to the lack of safety guarantees and reliability. The online learning setting is particularly difficult because real experience is tedious to obtain, due to safety and collision being of primary concern. While some works attempt to combat this problem through sim-to-real transfer techniques, the domain gap between simulation and reality is often too large to successfully deploy onto a real robot. In this work we demonstrate a learning system that is safe, efficient, and reliable while also having the ability to learn online on a real robotic platform to provide dynamic path planning for obstacle avoidance. The learning system leverages a fallback safety protocol to provide anti-collision guarantees as well as a learning signal, and generates reliable paths by integrating with a trajectory search method that provides structure to the overall learned behavior. We show results on our robotic platform for the task of obstacle avoidance during goal navigation, demonstrating a large improvement in search efficiency, task performance, and generalization when comparing to the baseline methods.

==> sections/old_baylearn.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Mobile robots are becoming more prevalent in humans' daily lives, performing tasks like vacuum cleaning, video recording, companionship, securities, etc.  Furthermore, due to advances in artificial intelligence and robotics, functionalities among robots are getting more comprehensive and autonomous. In this extended abstract, we focus on an essential factor - safety. For example, obstacle avoidance is critical for the safety of mobile robots, to avoid potential damage to humans, pets, or furniture. Therefore, we aim to design an efficient and safe system for mobile robots in dynamic real-world environments. 



A common way to ensure worse-case safety for real-world robots is deploying an Automatic Emergency Braking (AEB) system. 
%The AEB system provides maximum braking when there are obstacles or emergent situations.
Nonetheless, the AEB system could make overly simplified and sub-optimal decision that can result in head-on collision even though a steer maneuver could avoid it. 
%In addition, the AEB system can often make navigating the environment a non-smooth endeavor, and can at times be an inefficient compromise for safety having a negative affect on the user experience.  
A better way to ensure safety could be by allowing the robot to plan ahead to evaluate more options, before getting into a situation where an AEB system takes over. Another popular approach is to formulate collision avoidance as one of the cost terms in an overall search or trajectory optimization problem. With unlimited computation and/or if the problems are convex, such approach has hope for getting collision-free optimal solutions. Yet, in the typical settings for mobile robots, safety is often compromised against other goals in the overall optimization problem as most realistic planning problems are non-convex and NP-hard, with difficult dynamic and kinematic constraints as well \cite{lavalle2006planning}. 
In our work, we deploy a Reinforcement-Learning-guided (RL-guided) search~\cite{silver2016mastering} with real-world learning for robotics~\cite{haarnoja2018soft}. Our approach does in-time motion planning by learning to search for the optimal alternative trajectories, before it gets into an unsafe position where maximum braking is the only solution. 
%We also design the system in such a way where learning is done safely and collision free, even before the RL agent makes progress in the learning cycle. 
Our learning method also supports multi-robot interaction, which means the distributed learning system can be trained by having multiple robots safely operating in an common environment simultaneously, even in the presence of other humans. While there is related literature on safe RL, such as constrained policy optimization (CPO)~\cite{achiam2017constrained}, there is no guarantee that it can work in the real world. Our system works directly in the real world, and is able to provide safety guarantees during both the training and the inference cycles. 



Next, we discuss the challenge of deploying safety systems in the real world. A potential way is to design a safety module in simulation~\cite{wenzel2021vision} and then perform the sim-to-real transfer~\cite{zhao2020sim}. Nonetheless, the domain gap is enormous between simulation and the real world; more importantly, most simulation environments are static, but the real world is dynamic (keeps changing). Therefore, the real-world safety module must be adaptable to environmental changes. Another critical challenge is the diverse obstacles in the real world, including walls, moving objects (humans), glasses, etc. We consider a fusion strategy from heterogeneous sources of inputs, including Lidar, ultrasonic scanners, and wheel odometry, to tackle this challenge. These inputs complement each other: Lidar point clouds from Lidar scanners provide precise location information of obstacles but fail when there's a transparent substance such as glasses; sound waves from ultrasonic are noisier but can work with glasses; wheel odometry controls robot's states, such as velocity and acceleration.  One critical benefit of learning in the real-world is that we can speed up the search algorithm for planning with prior experiences encoded in the RL policy. During run time, every safety situation is being searched and solved as fast and optimal as possible, guided by the best heuristics learned in the presence of real-world situations and challenges. 


%In summary, we present a safety system in robots with four core properties: 1) it is efficient by performing an in-time path planning, 2) it performs learning and inference in the real world with a safety guarantee, 3) it allows multi-robot interactions, and 4) it handles a diverse set of obstacles by considering a multi-sensor fusion from inputs. 
Our experiments show that, when compared to the baseline methods (mobile robots without safety system and mobile robots with safety system using traditional trajectories search method), our approach enjoys higher average speed, lower crash rate, higher goals reached rate, lower computation, and still smooth overall trajectory. In a nutshell, we believe this work opens up a new horizon for designing real-world safety systems and thus accelerates the development of mobile robots autonomy. 


{\bf Our Approach.} At a high level, we present an auxiliary system to our robots for 1) collision avoidance and 2) in-time path planning in complex environments, including objects, humans, and glass/reflective surfaces. Our auxiliary system is a bypass system from the main robots system, and it only takes over the robots when it determines an unsafe situation. The correction actions include changing forwarding directions, reducing speed, and deploying maximum braking when a collision is almost happening. We note that, since our system is a bypass system, our collision avoidance is different from prior arts that consider reducing collision as one of the goals in a singular motion planning system~\cite{kahn2018self}. Prior designs aim to find a balance between safety and motion-planned goals; either safety or motion-planned goals can be compromised.

Our algorithmic design considers inputs from multiple sensors, including lidar, ultrasonic, and wheel odometry, to take care of glass detection and navigation in non-illuminated rooms. Then, our system calculates the trajectory of our robots, determining whether our robots are safe or unsafe. If our robot is in a safe position, the robot continues upstream control. On the other hand, if our robot is in an unsafe position, our system takes over the control: it applies a learning-based search to alter the robot trajectory (if possible) or perform maximum braking (if no good new trajectories are provided).  

Our search algorithm considers adding learnable parameters in Dynamic Window Approach (DWA)~\cite{fox1997dynamic} to speed up the search by reducing its exhaustive search space. The learning follows a real-world reinforcement learning setting: we put multiple robots in the real world, set up goal navigation tasks with random location goals, collect experiences and rewards, and update our system using Soft Actor-Critic (SAC)~\cite{haarnoja2018soft}. Our reward function considers three factors: 1) the size of the search space, 2) whether the trajectory leads us to an unsafe position, and 3) whether the location goal is reached.  

{\bf Experiments.} Our learning and evaluation are performed in real-world indoor environments, i.e. office spaces. The obstacles include non-moving objects and moving objects, such as humans (humans in the loop) and other moving robots. We consider two baselines for our method. The first baseline is a robotic setup in which we have the ability to map, localize, and navigate in an environment given goal locations. There is no safety system for this baseline. The second baseline adds our safety system onto the robots, but instead of having a learn-able search algorithm, we adopt DWA~\cite{fox1997dynamic} for performing the search for more optimal trajectories. After training, we evaluate all methods using goal navigation with $50$ random goals. We consider metrics to be 1) average speed of the robot, 2) crash rate, 3) goals reached, 4) search space (computation), and 5) unsmoothness (measured using averaged lateral velocity). 


We present the results in Table~\ref{tbl:comparisons} and shorthand the first baseline method as $\mathsf{baseline}$, the second baseline method as DWA-like traditional search method, and our method as $\mathsf{Ours}$. First, we compare $\mathsf{baseline}$ and traditional search. Their difference is considering a safety system or not. We observe that, with our safety system, traditional search achieves a much lower crash rate than $\mathsf{baseline}$, resulting in higher goals reached rate. Nonetheless, since traditional search includes an extensive search for alternative trajectories when in unsafe situations, it costs much more computation. Furthermore, we have large reduction in crash rate without large sacrifice in smoothness and average speed. This indicates our safety system does not have many false activation. Next, we compare traditional search and $\mathsf{Ours}$, with the difference being that the latter considers learning to search. We observe that all metrics except smoothness improve significantly. This fact suggests the effectiveness and the applicability of our method to the real world. Our next step is improving our system by considering smoothness into our RL reward function.  



==> sections/removed_content_from_main_text.tex <==
\input{fig_tex/reward_train}


\underline{\it Reward Function.} 
{\color{blue} I can work on this paragraph}
We also consider the Pure Reinforcement Learning baseline to demonstrate the effectiveness of our combined approach compared to a direct RL policy. The Pure Reinforcement Learning approach suffers greatly when it comes to collision rate, goals reached rate, and smoothness due to the lack of structure and safety guarantees in the learning and inference. It also achieves a much lower reward during the training cycle as shown in Fig.~\ref{fig:reward_train}.

==> tbl_tex/generalization.tex <==
\begin{table*}[t!]
\vspace{-1mm}
\centering
\caption{\small Quantitative comparisons in the evaluation environment.}
\vspace{-2mm}
\scalebox{1.0}{ \begin{tabular}{c|cc|cccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Search} &  Learning from  & average  & collisions ($\downarrow$) & \# max & latency ($\downarrow$) & search & unsmoothness ($\downarrow$) \\ && AEB & speed ($\uparrow$) & & braking ($\uparrow$) & & size ($\downarrow$) \\
\midrule
NoSafety  & no &  no &      0.41 m/s        &   16   &  n/a   & n/a     &   n/a    &    0.27 %m/s$^2$             
\\ 
AEB & no & no &       0.28 m/s        &    3    & 31  &  \textbf{8ms}   &     n/a  &     0.33                  
\\ 
DWA & yes & no &       0.37 m/s        &    1   & 9  &  100ms    &     2500       &     0.19                  
\\ 
RL  & no & yes &       0.42 m/s        &    5     & 7 &  15ms   &    n/a       &     0.26                  
\\
Ours & yes & yes &        \textbf{0.45 m/s}       &   \textbf{0}    & \textbf{4}  &   20ms   &  \textbf{25}    &   \textbf{0.16}                       
\\ \bottomrule
\end{tabular}
}
\label{tbl:generalization}
\vspace{-5mm}
\end{table*}

==> tbl_tex/old_malicious.tex <==
\begin{table*}[t!]
\vspace{-1mm}
\centering
\caption{\small Intentional Collision Attempts by Human Operator in Test Environment.}
\vspace{-2mm}
\scalebox{1.0}{\begin{tabular}{c|ccccc}
\toprule
{Method} & avg. speed & collisions & \# max braking & unsmoothness & avg. action cost \\
\midrule
AEB  & 0.31 m/s & 5 & 19 & 0.37 &  0.47     
\\ 
DWA & 0.43 m/s & 2 & 7 & 0.22 &  0.33         
\\ 
RL & 0.39 m/s & 3 & 9 & 0.49 &  0.35    
\\ 
Ours & 0.50 m/s & 0 & 3 & 0.14 & 0.21              
\\ \bottomrule
\end{tabular}
}
\label{tbl:random}
\vspace{-5mm}
\end{table*}

==> tbl_tex/old_table.tex <==
\begin{table*}[t!]
\centering
\caption{\small Quantitative comparisons in the training environment.}
\vspace{0mm}
\scalebox{1.0}{ \begin{tabular}{c|cc|cccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Search} &  Learning from  & average  & collisions ($\downarrow$) & \# max & latency ($\downarrow$) & search & unsmoothness ($\downarrow$) \\ && AEB & speed ($\uparrow$) & & braking ($\uparrow$) & & size ($\downarrow$) \\
\midrule
NoSafety & no &  no &      0.47 m/s        &  14   & n/a. & n/a & n/a  & 0.23 %m/s$^2$             
\\ 
AEB & no & no &       0.31 m/s        &    4    & 27 & \textbf{8 ms} &     n/a   &     0.31 %m/s$^2$                  
\\ 
DWA & yes & no &       0.44 m/s        &   2   & 7 & 100 ms &     2500    &     0.16 %m/s$^2$                  
\\ 
RL & no & yes &       \textbf{0.53 m/s}        &    3  &  8  &  15 ms &    n/a   &     0.27 %m/s$^2$                  
\\
Ours & yes & yes &        0.51 m/s       &  \textbf{1}   & \textbf{3} & 20 ms  &   \textbf{25}   &   \textbf{0.12} %m/s$^2$                       
\\ \bottomrule
\end{tabular}
}
\label{tbl:comparisons}
\vspace{-3mm}
\end{table*}
